Latent Mutants: A large-scale study on the Interplay between mutation testing and software evolution

In this paper we apply mutation testing in an in-time fashion, i.e., across multiple project releases. Thus, we investigate how the mutants of the current version behave in the future versions of the programs. We study the characteristics of what we call latent mutants, i.e., the mutants that are live in one version and killed in later revisions, and explore whether they are predictable with these properties. We examine 131,308 mutants generated by Pitest on 13 open-source projects. Around 11.2% of these mutants are live, and 3.5% of them are latent, manifesting in 104 days on average. Using the mutation operators and change-related features we successfully demonstrate that these latent mutants are identifiable, predicting them with an accuracy of 86% and a balanced accuracy of 67% using a simple random forest classifier.

==> bisection_study.tex <==
\section{Application in finding fault-inducing commits}

... % explin how these muatnst 

Section xxx shows that there are ... % ineterin gmust
We investigate whether existing tools of findiing fault-idncuign commits can effectively identify the injected commits.

% Also, how it differe from the bugs studied in these tools 


\subsection{Bisection}

\subsubsection{Git-bisection}

\subsubsection{Fonte}

\subsection{Results}

% table of fonte resutlts 

% the complexity of these mutans (level, paricufally, that gone thrroguh hchange ro not), the mutation oeprators (for this check whether they have different distrbution with thoes that often appeared in itneresitn gmutants)


% here, the best is to 
% some semantic analysis on the mutants that failed to be revaled by Fonte? e.g.. how natural this mutant is or soemthing like that



% small model (just to check whether it is classifialbe) that classify the mutants based on its likelihood to be interesting 

==> cluster_model.tex <==
% here, the best is to 


% some semantic analysis on the mutants that failed to be revaled by Fonte? e.g.. how natural this mutant is or soemthing like that

==> discussion_bic.tex <==
\section{RQ4.} % (fold)
\label{sec:rq4_}



\subsubsection{RQ4. Application study: bug-inducing commit study}

Q. how effective an existing tool is 

% the Usefulness of revealed mutants in Evaluating existing bug-inducing commits  

    % how this relate to the reported performace of the model 

Compare the performane of Fonte and a simple bisection on the effectiveness of locating mutant-injected commit. 
acc@n comparison, wef, since the target is limited 


There are cases where the injection completely remove the line -> deletion => for these cases, .. currently, excldued because it is ambgiuous to define the injection point (e.g., how mnay lines before and after)

\noindent\textbf{Bug Inducing Commit Identification}. 

%The root cause of software failure may not be among the recent changes that developers made. 
The software failure may be incurred by the previous changes that developer made rather than among the changes that developer make right before the failure.  
Recent studies [xxx] in software debugging thereby focus on identifying the commits that introduce changes that induce faults, which result in the observed failure. This additional information of bug-inducing commits can help developers understand the root cause of failures by providing the richer information of the source of failure along with xxx. 
One issue with this bug-inducing commit identification is the lack of a dataset to study. Identifying the ground-truth of bug-inducing commits is a trick task as ... % the source not clear etc. 

In this work, we study the impact of the propagation of mutants that are survived when they were first introduced, mainly investigating on the revelation of them in future. 
We thereby argue that the mutants revealed through subsqeuent changes can be used as the alternative dataset for bug-incducing commit identificaiton. 
\fixme{some benefits of this artificial dataset}{}
One main benefit of using such aritificial dataset is that we can now clearly know the bug-inducing commits of observed failures. 
To demonstrate the usefulness of revealed mutants, we investigate the performance of the state-of-the-art bug-inducing commit identification technique, Fonte, on identifying commits where the mutants are injected.

\noindent\textbf{Fonte.} Fonte is xxxx. 

In addition to the above method, we also apply the git-bisection technique, which was used as the baseline for Fonte to evaluate the weighted bisection by Fonte. 

Here, our foucs is the performace and whether the general idea remains the same 




\subsection{RQ4. Application study: bug-inducing commit study}

% the Usefulness of revealed mutants in Evaluating existing bug-inducing commits  
    % how this relate to the reported performace of the model 


\textbf{Answer to RQ4.} Performance slightly degrades, but the general trend remains the same. 


\begin{table}[ht] 
\caption{Subject of Bug-inducing commit identification. 
}\label{tab:tab3_revealed_mutants}
\scalebox{0.8}{
\begin{tabular}{l|rr|rr|rrrrr}
\toprule
 &  &  &  &  & \multicolumn{5}{c}{\# per category (\% \#$^{proc, cat}_{mut}$ over \#$^{proc}_{mut}$)}\\
proj & \#$^{all}_{rev}$ & \#$^{proc}_{rev}$& \#$^{all}_{mut}$ & \#$^{proc}_{mut}$ (\%) & \#$_{sc\_c}$ & \#$_{sc\_nc}$ & \#$_{rc\_c}$ & \#$_{rc\_nc}$ & \#$_{nc\_nc}$ \\
\midrule
Lang & 4 & 2 & 39 & 5 (12.82) & 0 (0.0) & 0 (0.0) & 3 (60.0) & 0 (0.0) & 2 (40.0)\\
Math & 7 & 7 & 77 & 33 (42.86) & 2 (6.06) & 4 (12.12) & 0 (0.0) & 0 (0.0) & 27 (81.82)\\
Cli & 1 & 1 & 2 & 2 (100.0) & 0 (0.0) & 0 (0.0) & 0 (0.0) & 0 (0.0) & 2 (100.0)\\
Compress & 15 & 13 & 78 & 70 (89.74) & 1 (1.43) & 10 (14.29) & 0 (0.0) & 1 (1.43) & 58 (82.86)\\
Codec & 6 & 5 & 19 & 15 (78.95) & 2 (13.33) & 5 (33.33) & 0 (0.0) & 0 (0.0) & 8 (53.33)\\
JacksonCore & 3 & 3 & 41 & 41 (100.0) & 0 (0.0) & 0 (0.0) & 2 (4.88) & 1 (2.44) & 38 (92.68)\\
Jsoup & 5 & 4 & 18 & 17 (94.44) & 3 (17.65) & 0 (0.0) & 0 (0.0) & 0 (0.0) & 14 (82.35)\\
\midrule
Total & 5 & 35 & 274 & 183 (66.79) & 8 (4.37) & 19 (10.38) & 5 (2.73) & 2 (1.09) & 149 (81.42)\\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[ht] 
\caption{Effectiveness of Fonte on identifying mutant-injected commits (i.e., artificial bug-inducing commits)
}\label{tab:tab3_revealed_mutants}
\scalebox{0.8}{
\begin{tabular}{lr|rr|rr|rr|rr|rr|rr}
\toprule
%& & \multicolumn{3}{c|}{All} & \multicolumn{3}{c|}{sc\_c} & \multicolumn{3}{c|}{sc\_nc} & \multicolumn{3}{c|}{rc\_c} & \multicolumn{3}{c|}{rc\_nc} & \multicolumn{3}{c}{nc\_nc} \\
% & & acc@ & &  & acc@ &  &  & acc@ &  &  & acc@ &  &  & acc@ &  &  & acc@ &  &  \\
%proj & \# & 1/5/10 & wef & MRR & 1/5/10 & wef & MRR & 1/5/10 & wef & MRR & 1/5/10 & wef & MRR & 1/5/10 & wef & MRR & 1/5/10 & wef & MRR \\
& & \multicolumn{2}{c|}{All} & \multicolumn{2}{c|}{sc\_c} & \multicolumn{2}{c|}{sc\_nc} & \multicolumn{2}{c|}{rc\_c} & \multicolumn{2}{c|}{rc\_nc} & \multicolumn{2}{c}{nc\_nc} \\
 & & acc@ & & acc@ &  & acc@ &  & acc@ &  & acc@ &  & acc@ &  \\
proj & \# & 1/5/10 & MRR & 1/5/10 & MRR & 1/5/10 & MRR & 1/5/10 & MRR & 1/5/10 & MRR & 1/5/10 & MRR \\
\midrule
Lang & 5 & 0/3/5 & 0.16 & (--/--/--) & --  & (--/--/--) & --  & 0/3/3 & 0.2 & (--/--/--) & --  & 0/0/2 & 0.1\\
Math & 33 & 0/0/0 & 0.019 & 0/0/0 & 0.03 & 0/0/0 & 0.027 & (--/--/--) & --  & (--/--/--) & --  & 0/0/0 & 0.017\\
Cli & 2 & 0/1/1 & 0.262 & (--/--/--) & --  & (--/--/--) & --  & (--/--/--) & --  & (--/--/--) & --  & 0/1/1 & 0.262\\
Compress & 70 & 0/16/38 & 0.108 & 0/0/1 & 0.167 & 0/0/5 & 0.087 & (--/--/--) & --  & 0/0/1 & 0.125 & 0/16/31 & 0.111\\
Codec & 15 & 0/0/0 & 0.061 & 0/0/0 & 0.053 & 0/0/0 & 0.053 & (--/--/--) & --  & (--/--/--) & --  & 0/0/0 & 0.069\\
JacksonCore & 41 & 0/7/13 & 0.106 & (--/--/--) & --  & (--/--/--) & --  & 0/2/2 & 0.2 & 0/0/0 & 0.033 & 0/5/11 & 0.103\\
Jsoup & 17 & 0/8/11 & 0.147 & 0/0/2 & 0.099 & (--/--/--) & --  & (--/--/--) & --  & (--/--/--) & --  & 0/8/9 & 0.157\\
\midrule
Total & 183 & 0/35/68 & 0.094 & 0/0/3 & 0.079 & 0/0/5 & 0.066 & 0/5/5 & 0.2 & 0/0/1 & 0.079 & 0/30/54 & 0.096\\
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figure/fonte_bisection.pdf}
  \caption{Bisection. sc-c, sc-nc, rc-c, rc-nc, nc-nc
  Total | (96/63/24) | (3/7/0) | (5/6/8) | (3/0/0) | (0/2/0) | (85/48/16)
  }
  \label{fig:rq4_biseciton}
\end{figure}



% section rq4_ (end)

==> methodology_terms.tex <==
\section{Methodology and Definition of Terms} % (fold)
\label{sub:definition_of_terms}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth, trim = 10mm 0mm 0mm 0mm]{figure/mutant_propagation.pdf}
  \caption{Mutant propagation example. Surviving mutants at $t_1$, $M_2$, $M_3$ and $M_4$, are propagated to the next versions. 
  Red and blue denote the deletion and the refactoring of code; green refers to semantic changes to the file. $M_2$ is revealed by a new test case at $t_3$, $M_4$ is deleted at $t_2$ and $M_3$ remains undetected to the end. 
  }\label{fig:mutant_propagation}
\end{figure}

\subsection{Mutant Propagation} % (fold)
\label{sub:mutant_propagation}
%\subsection{Key Insight}
% 1 to 11 yesers, median 90 days 
%\todo{Existing research on software debugging shows that there is a delay between the introduction and the revelation of faults\todo{~\cite{Cbabral2019icse}}. These faults that are later revealed are called \textit{latent} faults. Latent faults can occur for various reasons. Such examples include insufficient testing due to the premature understanding of the code around the faults. Thus, as the software matures/evolves, the existence of the latent faults are detected. Mutation testing tests the program by introducing artificial faults (i.e., mutants) that mimic faults in real-world. The usefulness of mutation testing to support software testing and debugging activities, especially in the absence of the ground truth faults, has been shown in many previous studies. Hence, we posit that similar to real-world faults, there exist latent mutants that are revealed in later versions of the program.  ... To check the existsence of latent mutants and their usefulness, we conduct a small study with the real-faults in Defecsts4J. xxxxx (briefly explain). From this study, we observe that around 24.8\% of the studied fautls (82 out of 357) have at least on latent fault that  ... }
In this study, we propagate surviving mutants of the present into future versions/commits of a program. %The key intuition behind this propagation is that latent mutants are coupled with latent faults in the code and thus will be revealed by future tests that detect the coupled faults. During this propagation. 
Previous studies show that latent faults are captured by future tests as they underwent various changes during the evolution of a program\todo{~\cite{}}. Since latent mutants are coupled with latent faults, we posit that similar relations between the software evolution and the mutants may also hold.  

%the same will likely hold for the latent mutants. 
\cref{fig:mutant_propagation} illustrates %how the software evolution can interact with the propagated mutants. 
an example of such interplay between propagated mutants and code evolution. Among the four mutants injected at $t_1$, $M_2$, $M_3$, and $M_4$ are undetected, i.e., surviving, by the test cases of a given time. At $t_2$, the line where $M_4$ is located is deleted, discarding $M_4$ from further inspection; the mutated lines of $M_2$ and $M_3$ are refactored (i.e., blue) here, but these two stay uncaught by the test cases at $t_2$. At $t_3$, $M_2$ is revealed by a new test case; while $M_2$ is not directly changed, it manifests due to its dependency on the changed lines (i.e., orange). The mutated line of $M_3$ is semantically changed at $t_4$. Still, the test cases at $t_4$ fail to detect $M_4$, resulting in $M_4$ surviving to the end.


\subsection{Definition of Terms} % (fold)
\label{sub:definition_of_terms}

In \cref{fig:mutant_propagation}, we observe three different mutant states after the propagation. This section defines different categories of mutants based on these three mutant propagation states and the initial mutation testing results.

\noindent
\textbf{Killed Mutants: } A mutant is \textit{killed} if there exists \textit{at least} one test case (in the software's test suite) which \textit{reveals the fault} \textit{mimicked} by the mutation. %We say that a test case reveals the fault if it is sufficient to distinguish the observable behavior between the mutant and the original program.  
The goal of mutation testing is to kill all mutants. The number of killed mutants is employed to measure the adequacy of the test suite. \fixme{Consider \autoref{fig:mutant_propagation} with \textit{four} injected mutants $\{M_1, M_2,  M_3,  M_4\}$. In this example, mutant $M_1$ is \textit{killed} at time $t_1$. Thus, we say that the \textit{mutation score} at time $t_1$, computed as the ratio of killed mutants over the total number of generated mutants, is \checknumber{0.25}.}{} % do we mention mutation score here? 

\vspace{0.5mm}
\noindent
\textbf{Live Mutants:} This refers to the mutants that remain undetected (i.e., \textit{not killed}) by the existing test suite, i.e., no test case in the current test suite distinguishes the behaviour of the mutants from that of the original program. \autoref{fig:mutant_propagation} shows that three mutants ($M_2,  M_3$ and  $M_4$) \textit{are live} at time $t_1$.\footnote{We call these initial surviving mutants as live to further differentiate with the mutants that survive after the propagation.} 

%\vspace{0.5mm}\noindent\textbf{Propagated Mutants:} In this work, we \textit{propagate} \textit{live mutants} by injecting these mutants into future program versions. %\autoref{fig:mutant_propagation} shows that the two surviving mutants ($M_2,$ and $M_3$) injected in the program version at time $t_1$ were successfully propagated into a future version of the program at time $t_2$. In \autoref{fig:mutant_propagation}, $M_2$, $M_3$, and $M_4$ are propagated mutants, each with a different final state.  
\vspace{1mm}
We \textit{propagate} \textit{live mutants}, introducing them to future program versions. In \autoref{fig:mutant_propagation}, $M_2$, $M_3$, and $M_4$ are propagated, each of them belonging to a different group with a different final state.

\vspace{1mm}
\noindent\textbf{Latent Mutants} 
%fault revealing mutation testing is to generate mutants that lead to test cases which reveal faults in the program under test.  For instance,  we say that mutant  $M_1$ is a fault revealing mutants if it leads to the generation of a test suite that reveals a \textit{real fault} in the program.  \todo{concretely, how does this relate to latent mutants?}
The mutant that failed to be captured by the current test suite but caught by the future test suite belong to this category. We call these mutants \textit{latent mutants} similar to the naming of latent faults. In \cref{fig:mutant_propagation}, $M_2$ is a \textit{latent mutant} since it is killed by tests at $t_3$ but not by those at $t_1$. 
%In this work, we investigate if \textit{surviving mutants} injected at time $t_1$ are \textit{killed} (i.e., reveal faults) in the future, i.e., at time $t_{1+i}$. We refer to such mutants as \textit{latent mutants}. Consider \autoref{fig:mutant_propagation}, mutant $M_2$ is a \textit{latent mutant} because it was injected at time $t_1$ and \textit{survived}, but it is \textit{killed} in the future, i.e., time $t_3$. 

\noindent
\textbf{Non-latent Mutants:} Non-latent mutants denote the mutants that are killed by none of the future test suites during the propagation. Consider \autoref{fig:mutant_propagation}, mutant $M_3$ is a \textit{non-latent mutant} because it was injected at time $t_1$ and was never killed to the end, $t_4$. We call them non-latent since there is no evidence that supports these mutants to be useful for future testing. 


\noindent
\textbf{Discarded Mutants:} %In this paper, a \textit{propagated mutant} is \textit{dead} if it is deleted or overwritten in future versions. This is due to code evolution, i.e., code refactoring or implementation of new features between both program versions. Thus, dead mutants have no impact on the future version of the program since they are not part of the executable code base. \autoref{fig:mutant_propagation} shows that mutant $M_4$ is a \textit{dead mutant} in program version at time $t_2$ because it is located on a deleted program component (red portion of the program). % due to code refactoring.}
This refers to mutants deleted or overwritten by developers and thus discarded from further inspection. %; code refactoring or implementation of new features between both program versions can be the reason. 
Discarded mutants have no impact on the future version of the program since they no longer exist in the executable code base. In \autoref{fig:mutant_propagation}, mutant $M_4$ is a {discarded mutant} in the program version at $t_2$ because it is located on a deleted program component (red).

\subsection{Code Evolution and Mutant Propagation} % (fold)
\label{sub:code_evolution_and_mutant_propagation}

Software evolves through the changes made by developers; some of them change the program semantics, some only the syntax, and even limited to the style changes. Thus, as depicted in \cref{fig:mutant_propagation}, mutants will likely undergo various changes as they propagate to future versions. To study how the change type affects the final mutant state, mainly their disclosure, we differentiate changes on the mutated lines into three: 1) semantically changed, 2) refactored, and 3) not changed; the last one includes white space and comment changes, as these changes impact neither the syntax nor semantic of the code. The latent mutants can be revealed either by the changes directly made on them or by the changes on dependent code (e.g., the case of $M_2$ in \cref{fig:mutant_propagation}). Combined with the three initial change groups we defined, we categorise latent mutants further into five categories. 

\begin{itemize}
  \item $SC_{C}$. Semantically changed and revealed by changes on the mutated line 
  \item $SC_{NC}$. Semantically changed and revealed by changes on the dependent lines
  \item $RC_{C}$. Refactored and revealed by changes on the mutated line 
  \item $RC_{NC}$. Refactored and revealed by changes on the dependent lines
  \item $NC_{NC}$. Not changed and revealed by changes on the dependent lines
\end{itemize}

%The \textit{mutated line} refers to th e

Different changes can be made on the mutated line. For this categorisation of latent mutants, we consider the line \textit{semantically changed} if it was semantically changed even once; we regard the line to be refactored if it only went through code refactorings. Regarding the mutant revelation through the changes on the dependent code, we consider only the changes in the same file. 
%For the dependency between lines, we ..(-> we do not inspect deeply by actually generating the dependency graph (can be future work?)) only limited to the lines within the same file; the mutant check is done if and only if the mutated files is changed (-> threat to validity?) 


% subsection software_evolution (end)

% section background (end)


==> result_analysis.tex <==
\section{Results}\label{sec:result_analysis}


\subsection{RQ1. Mutant Survival and Kill} % (fold)
\label{sub:rq1_mutant_surival_and_killed}

\begin{table}[ht] 
\caption{Initial mutation testing results. Others includes No coverage, Time out, Non viable, Memory error, and Run error. 
\textit{avg} refers to the average across revisions within the project, and \textit{total} is computed without differentiating revisions. The values in the last row, \textit{Total}, are calculated using all generated mutants. 
}\label{tab:tab1_init_mut_stat}
\scalebox{0.7}{
\begin{tabular}{lr|rr|rr|rr|rr} %|rr}
    \toprule
     & & \multicolumn{2}{c|}{All} & \multicolumn{2}{c|}{Live (\%)}  & \multicolumn{2}{c|}{Killed (\%)} & \multicolumn{2}{c}{Others (\%)} \\
Proj & \#$_{rev}$ & avg & total & avg & total & avg & total & avg & total \\
\midrule
Lang & 49 & 346.39 & 16973 & 8.18 & 7.12 & 56.4 & 56.04 & 35.42 & 36.84 \\
Math & 104 & 274.5 & 28548 & 11.74 & 10.05 & 65.93 & 61.31 & 22.33 & 28.63 \\
Time & 20 & 154.3 & 3086 & 9.62 & 8.85 & 83.7 & 84.54 & 6.67 & 6.61 \\
Closure & 139 & 244.38 & 33969 & 8.95 & 10.07 & 72.14 & 74.26 & 18.91 & 15.66 \\
Cli & 30 & 92.0 & 2760 & 8.94 & 9.93 & 86.16 & 85.25 & 4.91 & 4.82 \\
Compress & 45 & 186.02 & 8371 & 15.08 & 16.9 & 71.98 & 67.69 & 12.94 & 15.41 \\{}
Codec & 18 & 197.83 & 3561 & 11.64 & 10.11 & 80.74 & 83.46 & 7.62 & 6.43 \\
Collections & 2 & 218.0 & 436 & 11.63 & 14.91 & 28.1 & 19.72 & 60.26 & 65.37 \\
Csv & 14 & 102.36 & 1433 & 8.63 & 12.35 & 84.65 & 80.88 & 6.72 & 6.77 \\
JacksonCore & 22 & 888.0 & 19536 & 16.72 & 14.78 & 58.47 & 61.61 & 24.8 & 23.61 \\
JacksonXml & 3 & 99.33 & 298 & 7.89 & 8.39 & 56.16 & 55.37 & 35.95 & 36.24 \\
JxPath & 9 & 189.44 & 1705 & 10.33 & 9.21 & 72.64 & 72.43 & 17.02 & 18.36 \\
Jsoup & 92 & 115.57 & 10632 & 14.74 & 15.17 & 74.98 & 73.78 & 10.28 & 11.05 \\
\midrule
Total & 547 & 240.05 & 131308 & 11.33 & 11.23 & 71.02 & 67.3 & 17.64 & 21.47 \\
    \bottomrule
\end{tabular}}
\end{table} 


\cref{tab:tab1_init_mut_stat} shows the initial results of mutation testing. In total, 131,308 mutants are generated. Among them, 11.23\% of them (14747) remain undetected while 71.02\% are detected, i.e., killed, by failing test cases; remaining 21.47\% includes mutants killed by other factors, such as time-out, along with the mutants never been executed by test cases. The ratios vary depending on the projects but overall are similar. As we are interested in how the mutants executed but failed to be detected differs from those killed, we consider these mutants in \textit{Others} out-of-scope, focusing only on the mutants explicitly labelled as \textit{Surviving} and \textit{Killed}. 

\cref{tab:tab_rq1_surv_mutop,tab:tab_rq1_kill_mutop} show the proportion of surviving and killed mutants wwhen using each operator, respectively. The operator that leads to the highest ratio of surviving/killed mutant are highlighted in blue; those within the top five are highlighted in green; the last row, \textit{TotalFreq}, presents the frequency of mutators within the top five across projects. Overall, there are clear differences between these two groups of mutators. Overall, the mutators that result in undetected mutants in \cref{tab:tab_rq1_surv_mutop} a
Overall, the mutators that are less likely to change the initial program execution path tend to generate more mutants that are undetected by a test suite, as shown in \cref{tab:tab_rq1_surv_mutop}. In contrast, the mutators with a higher mutant-kill ratio are those that directly affect the execution path.
%For instance, Conditionals Boundary Mutator (CB) and Void Method Call (VMC), the top two regarding the survival rate, have more chance to maintain the original execution path of a program compared to the Negate Conditionals operator, which explicitly changes the execution path by negating the condition and thereby produces the highest mutant kill rate; CB also changes the conditional statements but make only subtle changes (e.g., $<$ to $\geq$). 
For instance, while both Conditionals Boundary Mutator (CB) and Negate Conditionals (NC) operators mutate the conditionals, CB that makes subtle changes on the condition boundary (e.g., $<$ to $\leq$) has the highest likelihood of surviving mutants whereas NC that explicitly changes the execution path by negating the condition results in the highest mutant kills. Similarly, the Void Method Call (VMC) operator, which removes method calls to void methods, is more likely to generate surviving mutants than mutators, such as Empty Returns (ERET), that mutate the method calls to non-void methods. These comparisons confirm the importance of the role of mutators on the mutant survivals and kills,  \fixme{conforming with the findings on .. }{cite} % JJ: not sure whether there are some studies that explicitly 

Previously in \cref{sub:rq1}, we conjecture that the past change tendency of mutated code may affect the detectability of mutants: for instance, does mutating the lines with more frequent changes lead to more frequent mutant kills and vice-versa? \cref{fig:rq1_chg} demonstrates the results of such analyses. The boxplots in this figure compare the eight historical metrics defined in \cref{sub:rq1} between surviving and killed mutants. The results vary depending on projects; in this paper, we present the results of two projects with two representative, common patterns observed across different projects. 
One of the most observed patterns is that killed mutants reside more often in the recently changed and introduced code, whereas for surviving mutants, the opposite holds (show in \cref{fig:rq1_lang_chg})\footnote{We observe a similar trend across four different projects; some have mixed trend of the opposite depending on the metric.}. In addition, mutants in the frequently changed lines tend to be more detected than those in rarely changed lines. These combined imply that mutating actively maintained code results in more killed mutants; we can suspect this to be related to more frequent testing by developers. 
However, we also frequently observe the opposite trend, as shown in \cref{fig:rq1_closure_chg} for Closure\footnote{Surviving mutants of around five projects often reside in the code that was recently changed or introduced compared to the killed mutants.} Here, mutating recently changed or introduced code leads to more surviving mutants. For this, we suspect the recent code has not yet been sufficiently tested, as opposite to the previously cases. For the number of developers, i.e., $n^l_{dev}$ and $n^e_{dev}$, the trend is less obvious. 
Nevertheless, despite having different trends, all projects show differences in the past change tendencies of code with surviving mutants and killed mutants. 

\noindent\textbf{Answer to RQ1.} Surviving mutants take around 10\% of generated mutants in total. Compared to killed mutants, these mutants are often generated with different mutation operators and reside in the code with different past change trends with the killed mutants within the projects. 


\begin{table}[ht] 
\caption{Mutators and Live Mutant. Each value is reported in the percentage of mutant survival when the mutator in the column is used: $\frac{n_{surv}}{n}$, $n$ is the number of mutants generated by the mutator 
Those with the highest ratios are in bold, and underlined means the operators to be within the top five operators with the highest ratio of survived mutants when used. 
}\label{tab:tab_rq1_surv_mutop}
\scalebox{0.7}{
\begin{tabular}{l|rrrrrrrrrrr}
    \toprule

\textit{Perc (\%)} & MATH & CB & INCR & IN & NC & VMC & PRET & ERET & BFRET & BTRET & NRET \\
\midrule

Lang & \cellcolor{green!25}13.1 & \cellcolor{blue!25}\textbf{32.4} & 1.2 & 3.1 & 2.2 & \cellcolor{green!25}6.3 & 5.0 & 1.5 & 0.0 & 1.9 & 0.8\\
Math & 8.9 & \cellcolor{blue!25}\textbf{31.6} & 1.1 & \cellcolor{green!25}10.3 & 6.0 & \cellcolor{green!25}16.5 & 3.5 & 0.9 & 6.1 & 9.6 & 0.3\\
Time & 10.9 & \cellcolor{blue!25}\textbf{30.8} & 8.1 & \cellcolor{green!25}19.4 & 6.4 & \cellcolor{green!25}13.3 & 1.0 & 4.6 & 2.6 & 7.7 & 5.2\\
Closure & 10.1 & \cellcolor{blue!25}\textbf{26.4} & 8.0 & 0.0 & 3.6 & \cellcolor{green!25}19.4 & 5.0 & 3.6 & 6.0 & 7.2 & \cellcolor{green!25}18.7\\
Cli & 14.3 & \cellcolor{blue!25}\textbf{41.6} & 4.3 & - & 2.6 & 8.8 & 4.3 & 3.7 & 5.3 & \cellcolor{green!25}16.7 & \cellcolor{blue!25}\textbf{41.6}\\
Compress & \cellcolor{green!25}17.1 & \cellcolor{blue!25}\textbf{42.2} & 6.0 & 0.0 & 9.4 & \cellcolor{green!25}24.6 & 12.5 & 15.3 & 8.2 & 7.9 & 0.8\\
Codec & \cellcolor{green!25}11.9 & \cellcolor{blue!25}\textbf{40.3} & 2.4 & - & 7.1 & 3.8 & 0.0 & \cellcolor{green!25}8.5 & 3.1 & 2.7 & 3.5\\
Collections & 14.3 & \cellcolor{green!25}30.4 & 0.0 & - & \cellcolor{green!25}18.3 & 10.7 & \cellcolor{blue!25}\textbf{50.0} & 12.5 & 0.0 & 9.1 & 8.6\\
Csv & \cellcolor{blue!25}\textbf{69.7} & \cellcolor{green!25}31.4 & 0.0 & - & 5.2 & \cellcolor{green!25}14.8 & 12.5 & 1.6 & 0.0 & 0.0 & 0.0\\
JacksonCore & \cellcolor{green!25}9.5 & \cellcolor{blue!25}\textbf{50.9} & 9.2 & 0.0 & \cellcolor{green!25}12.1 & 9.1 & 4.4 & 2.2 & 8.1 & 2.3 & 5.6\\
JacksonXml & 0.0 & \cellcolor{blue!25}\textbf{33.3} & 0.0 & - & 4.8 & 10.0 & 0.0 & 3.4 & 0.0 & \cellcolor{green!25}14.3 & \cellcolor{green!25}25.0\\
JxPath & \cellcolor{green!25}10.3 & \cellcolor{green!25}41.2 & 0.0 & - & 6.4 & \cellcolor{blue!25}\textbf{42.5} & 7.5 & 9.1 & 10.0 & 7.4 & 1.6\\
Jsoup & 10.7 & \cellcolor{blue!25}\textbf{38.4} & 1.5 & - & 5.3 & \cellcolor{green!25}30.4 & 9.7 & 4.1 & 10.0 & 9.9 & \cellcolor{green!25}23.0\\
\midrule
Total & 10.5 & \cellcolor{blue!25}\textbf{37.4} & 4.2 & 9.9 & 5.7 & \cellcolor{green!25}18.2 & 4.9 & 3.2 & 5.8 & 6.6 & \cellcolor{green!25}11.6\\
\bottomrule
TopFreq & \cellcolor{green!25}6 & \cellcolor{blue!25}\textbf{14} & 0 & 2 & 2 & \cellcolor{green!25}9 & 1 & 1 & 0 & 2 & 5\\
    \bottomrule
\end{tabular}}
\end{table} 


%Conditional bondary, Math, void method call -> harder to catch (void method call -> far more survived then method call with acutla return)


\begin{table}[ht] 
\caption{Mutators and Killed Mutant. Each value is reported in the percentage of mutant kill when the mutator in the column is used: $\frac{n_{kill}}{n}$, $n$ is the number of mutants generated by the mutator 
}\label{tab:tab_rq1_kill_mutop}
\scalebox{0.7}{
\begin{tabular}{l|rrrrrrrrrrr}
    \toprule
\textit{Perc (\%)} & MATH & CB & INCR & IN & NC & VMC & PRET & ERET & BFRET & BTRET & NRET \\
\midrule
Lang & 51.2 & 33.8 & 56.2 & 37.5 & \cellcolor{green!25}62.4 & 44.4 & \cellcolor{blue!25}\textbf{68.1} & \cellcolor{green!25}61.6 & 56.2 & 55.0 & 54.1\\
Math & 63.0 & 39.5 & \cellcolor{green!25}68.1 & \cellcolor{blue!25}\textbf{72.1} & 66.0 & 51.4 & 64.9 & 62.7 & 51.5 & 47.0 & \cellcolor{green!25}71.8\\
Time & 80.8 & 62.8 & 78.4 & 80.6 & \cellcolor{green!25}89.8 & 70.3 & \cellcolor{blue!25}\textbf{93.8} & 87.2 & 89.5 & 72.3 & \cellcolor{green!25}89.8\\
Closure & 78.3 & 58.3 & 71.7 & 31.6 & \cellcolor{green!25}83.0 & 62.5 & 51.7 & \cellcolor{green!25}82.9 & \cellcolor{blue!25}\textbf{83.1} & 79.5 & 66.6\\
Cli & 71.4 & 52.2 & 87.0 & - & \cellcolor{blue!25}\textbf{94.8} & 85.9 & 73.9 & \cellcolor{green!25}92.0 & \cellcolor{green!25}89.5 & 80.2 & 52.6\\
Compress & 68.0 & 47.8 & \cellcolor{green!25}89.7 & \cellcolor{blue!25}\textbf{100.0} & 78.5 & 56.6 & 54.9 & 61.0 & 42.4 & 53.2 & \cellcolor{green!25}86.2\\
Codec & 85.5 & 54.4 & 86.5 & - & 85.2 & \cellcolor{green!25}90.9 & \cellcolor{blue!25}\textbf{95.1} & 83.0 & 81.5 & 80.2 & \cellcolor{green!25}86.9\\
Collections & 7.1 & 8.7 & \cellcolor{blue!25}\textbf{66.7} & - & 18.3 & 7.1 & \cellcolor{green!25}50.0 & \cellcolor{green!25}62.5 & 33.3 & 18.2 & 23.4\\
Csv & 25.8 & 52.3 & 76.9 & - & 89.6 & 77.0 & 78.1 & \cellcolor{green!25}95.3 & \cellcolor{blue!25}\textbf{100.0} & 86.3 & \cellcolor{green!25}98.0\\
JacksonCore & 69.2 & 35.5 & \cellcolor{green!25}73.0 & \cellcolor{blue!25}\textbf{100.0} & \cellcolor{green!25}71.1 & 41.5 & 68.4 & 69.5 & 51.9 & 52.5 & 69.5\\
JacksonXml & 11.1 & 44.4 & \cellcolor{blue!25}\textbf{100.0} & - & \cellcolor{green!25}73.0 & 50.0 & 28.0 & 37.9 & \cellcolor{green!25}60.0 & 28.6 & 50.0\\
JxPath & 66.7 & 33.8 & 54.5 & - & \cellcolor{green!25}78.1 & 42.5 & 46.2 & 68.9 & \cellcolor{green!25}81.4 & 73.6 & \cellcolor{blue!25}\textbf{86.0}\\
Jsoup & 77.5 & 56.7 & \cellcolor{green!25}88.1 & - & \cellcolor{blue!25}\textbf{89.0} & 53.1 & 77.7 & \cellcolor{green!25}83.7 & 80.2 & 70.2 & 59.2\\
\midrule
Total & 65.8 & 41.6 & 71.8 & 70.7 & \cellcolor{blue!25}\textbf{76.2} & 57.5 & 64.3 & \cellcolor{green!25}73.8 & \cellcolor{green!25}75.1 & 70.3 & 67.5\\
\bottomrule
TopFreq & 0 & 0 & \cellcolor{green!25}6 & 3 & \cellcolor{blue!25}\textbf{9} & 1 & 4 & \cellcolor{green!25}7 & \cellcolor{green!25}6 & 0 & \cellcolor{green!25}6\\
\bottomrule
\end{tabular}}
\end{table} 


\begin{figure}[ht]
\centering
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq1/Lang_chg.pdf}
    \caption{Lang}
    \label{fig:rq1_lang_chg}
\end{subfigure}
\hfill
%\begin{subfigure}{0.3\textwidth}
%    \includegraphics[width=\textwidth, trim = 20mm 10mm 14mm 0mm]{figure/rq1/Compress_chg.pdf}
%    \caption{Compress} % Or Josup
%    \label{fig:rq1_compress_chg}
%\end{subfigure}
%\hspace{-5em}
%\hfill
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq1/Closure_chg.pdf}
    \caption{Closure}
    \label{fig:rq1_closure_chg}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq1/Total_chg.pdf}
    \caption{Total}
    \label{fig:rq1_total_chg}
\end{subfigure}
\caption{Closure, Time, Math similar patterns: i.e., killed longer lived, Others: i.e., killed more recently changed  %(overall, churn more frequent -> common)
White marks are the mean, and the red lines are the median. 
}\label{fig:rq1_chg}
\end{figure}



\subsection{RQ2. Revealed Mutants Characteristics} % (fold)
\label{sub:rq2_revealed_mutants_characteristics}

\begin{table}[ht] 
\caption{Mutant Propagation Status. \#$^{prop}_{rev}$ and \#$^{prop}_{mut}$ show how the number of revisions and propagated mutants change through preprocessing: from right to left, the numbers refer to those with at least one propagated live mutants, those replicated, and those remaining after the threshold of 365 days for the propagation status; %76.1\% and 57.3\% of non-latent and latent mutants remain after the filtering with the threshold. 
 %Out of 12,239 propagated mutants from, 10383 mutants (84.8\%) remain after the exclusion of mutants with the threshold of 365 days; 
With this threshold of 365 days, 76.1\% and 57.3\% of non-latent and latent mutants remain. 
\textit{average} is the average per revision, and \textit{agg} contains the aggregated value per project. 
The last row, \textit{Total}, contains the percentage computed with all generated mutants, and \textit{avg} per revision. 
}\label{tab:tab_rq2_mut_status}
\scalebox{0.65}{
\begin{tabular}{lrr|r|rr|rr|rr}
\toprule
%& & & & \multicolumn{2}{c|}{Revealed (\# (\%))} & \multicolumn{2}{c|}{Survived (\# (\%))} & \multicolumn{2}{c}{Dead (\# (\%))} \\
%proj & & \#$_{rev}$ & \#$_{mut}$ (avg.) & average & total & average & total & average & total \\
& \multicolumn{2}{c|}{\#$^{prop}_{rev}$} & \#$^{prop}_{mut}$ & \multicolumn{2}{c|}{Latent (\# (\%))} & \multicolumn{2}{c|}{Non-latent (\# (\%))} & \multicolumn{2}{c}{Discard (\# (\%))} \\
%proj & init & thr$_{365}$/valid/all &  & \#$_{mut}$ & average & total & average & total & average & total \\
%proj & \# & \#$^{v,365}_{w.l}$/\#$^{v}_{w.l}$/\#$^{w.l}$ & \#$_{mut}$ (avg.) & average & total & average & total & average & total \\
proj & \#$_{rev}$ & & \#$_{mut}$ & average & agg & average & agg & average & agg \\
\midrule 
Lang & 49 & \textbf{27}/30/33& \textbf{833}/1025/1209& 1.4 (9.4\%) & 39 (4.7\%) & 22.9 (72.3\%) & 618 (74.2\%) & 6.5 (18.3\%) & 176 (21.1\%)\\
Math & 104 & \textbf{79}/89/92& \textbf{1442}/2099/2870& 1.7 (6.0\%) & 136 (9.4\%) & 10.5 (63.1\%) & 831 (57.6\%) & 6.0 (30.9\%) & 475 (32.9\%)\\
Time & 20 & \textbf{10}/19/19& \textbf{79}/185/273& 0.5 (12.8\%) & 5 (6.3\%) & 7.3 (86.0\%) & 73 (92.4\%) & 0.1 (1.2\%) & 1 (1.3\%)\\
Closure & 139 & \textbf{100}/118/118& \textbf{2242}/2866/3421& 0.3 (4.0\%) & 33 (1.5\%) & 16.7 (68.0\%) & 1668 (74.4\%) & 5.4 (28.0\%) & 541 (24.1\%)\\
Cli & 30 & \textbf{22}/25/25& \textbf{232}/237/274& 0.5 (3.7\%) & 10 (4.3\%) & 8.4 (89.4\%) & 184 (79.3\%) & 1.7 (6.9\%) & 38 (16.4\%)\\
Compress & 45 & \textbf{43}/44/44& \textbf{1089}/1201/1415& 0.6 (3.4\%) & 26 (2.4\%) & 12.7 (58.7\%) & 544 (50.0\%) & 12.1 (37.8\%) & 519 (47.7\%)\\
Codec & 18 & \textbf{16}/16/18& \textbf{271}/282/360& 0.8 (2.6\%) & 13 (4.8\%) & 9.2 (54.8\%) & 148 (54.6\%) & 6.9 (42.6\%) & 110 (40.6\%)\\
Collections & 2 & \textbf{2}/2/2& \textbf{4}/4/65& 0.0 (0.0\%) & 0 (0.0\%) & 2.0 (100.0\%) & 4 (100.0\%) & 0.0 (0.0\%) & 0 (0.0\%)\\
Csv & 14 & \textbf{11}/11/12& \textbf{143}/152/177& 0.1 (9.1\%) & 1 (0.7\%) & 10.5 (63.1\%) & 115 (80.4\%) & 2.5 (27.8\%) & 27 (18.9\%)\\
JacksonCore & 22 & \textbf{21}/22/22& \textbf{2635}/2645/2888& 2.4 (1.2\%) & 51 (1.9\%) & 15.7 (37.6\%) & 330 (12.5\%) & 107.3 (61.2\%) & 2254 (85.5\%)\\
JacksonXml & 3 & \textbf{3}/3/3& \textbf{17}/17/25& 0.0 (0.0\%) & 0 (0.0\%) & 1.3 (26.7\%) & 4 (23.5\%) & 4.3 (73.3\%) & 13 (76.5\%)\\
JxPath & 9 & \textbf{9}/9/9& \textbf{135}/135/157& 0.0 (0.0\%) & 0 (0.0\%) & 13.6 (95.8\%) & 122 (90.4\%) & 1.4 (4.2\%) & 13 (9.6\%)\\
Jsoup & 92 & \textbf{79}/85/85& \textbf{1261}/1391/1613& 0.6 (8.7\%) & 50 (4.0\%) & 5.3 (41.6\%) & 415 (32.9\%) & 10.1 (49.7\%) & 796 (63.1\%)\\
\midrule
Total & 547 & \textbf{422}/473/482& \textbf{10383}/12239/14747& 0.9 (5.5\%) & 364 (3.5\%) & 12.0 (61.3\%) & 5056 (48.7\%) & 11.8 (33.1\%) & 4963 (47.8\%)\\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[ht] 
\caption{Mutation Operators and Latent Mutants. JxPath, Collections and JacksonXml are excluded as they no longer have any mutant left.
}\label{tab:tab_rq2_rv_mut_mutop}
\scalebox{0.7}{
\begin{tabular}{l|rrrrrrrrrrr}
    \toprule
\textit{Perc (\%)} & MATH & CB & INCR & IN & NC & VMC & PRET & ERET & BFRET & BTRET & NRET \\
\midrule 
Lang & \cellcolor{green!25}7.14 & 3.42 & \cellcolor{green!25}16.67 & 0.0 & 6.35 & \cellcolor{blue!25}\textbf{17.39} & 0.0 & 5.88 & - & 0.0 & 0.0\\
Math & 24.03 & 9.46 & \cellcolor{green!25}25.0 & \cellcolor{blue!25}\textbf{46.67} & \cellcolor{green!25}34.48 & 19.14 & 11.32 & 0.0 & 0.0 & 6.25 & 0.0\\
Time & \cellcolor{green!25}0.0 & \cellcolor{green!25}0.0 & - & - & \cellcolor{green!25}13.33 & \cellcolor{blue!25}\textbf{23.08} & \cellcolor{green!25}0.0 & \cellcolor{green!25}0.0 & - & \cellcolor{green!25}0.0 & -\\
Closure & 0.0 & 0.8 & 0.0 & - & \cellcolor{blue!25}\textbf{11.23} & 0.41 & \cellcolor{green!25}2.33 & \cellcolor{green!25}4.0 & 1.85 & 1.08 & 0.46\\
Cli & \cellcolor{green!25}7.69 & \cellcolor{blue!25}\textbf{9.59} & 0.0 & - & 0.0 & \cellcolor{green!25}2.63 & 0.0 & 0.0 & 0.0 & 0.0 & 1.39\\
Compress & \cellcolor{green!25}4.0 & 0.62 & 0.0 & - & \cellcolor{green!25}4.0 & 2.55 & \cellcolor{blue!25}\textbf{4.65} & 0.0 & 0.0 & 0.0 & 0.0\\
Codec & 2.04 & \cellcolor{green!25}6.0 & - & - & \cellcolor{green!25}8.33 & 0.0 & - & 0.0 & 0.0 & \cellcolor{blue!25}\textbf{33.33} & 0.0\\
Csv & \cellcolor{green!25}0.0 & \cellcolor{green!25}0.0 & - & - & \cellcolor{green!25}0.0 & \cellcolor{blue!25}\textbf{9.09} & \cellcolor{green!25}0.0 & - & - & - & -\\
JacksonCore & 0.62 & 2.0 & 1.23 & - & \cellcolor{green!25}2.83 & 0.43 & \cellcolor{green!25}2.94 & \cellcolor{blue!25}\textbf{16.67} & 0.0 & 0.0 & 2.7\\
Jsoup & 2.9 & 3.72 & 0.0 & - & 6.9 & 3.47 & 0.0 & \cellcolor{blue!25}\textbf{17.39} & \cellcolor{green!25}16.0 & \cellcolor{green!25}10.64 & 1.27\\
\midrule
Total & \cellcolor{green!25}11.03 & 3.95 & 3.08 & \cellcolor{blue!25}\textbf{45.65} & \cellcolor{green!25}8.06 & 2.83 & 4.48 & 7.29 & 4.81 & 3.94 & 0.88\\
\bottomrule
TopFreq & \cellcolor{green!25}6 & 4 & 2 & 2 & \cellcolor{blue!25}\textbf{8} & 4 & \cellcolor{green!25}5 & 4 & 1 & 3 & 0\\
\bottomrule
\end{tabular}}
\end{table} 

\begin{figure}[h]
\centering
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_CONDITIONALS_BOUNDARY.pdf}
    \caption{CB}
    \label{fig:rq2_CB}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_VOID_METHOD_CALLS.pdf}
    \caption{VMC}
    \label{fig:rq2_VMC}
\end{subfigure}
%\hspace{-5em}
\hfill
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_MATH.pdf}
    \caption{MATH}
    \label{fig:rq2_MATH}
\end{subfigure}
%\hspace{-5em}
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_NEGATE_CONDITIONALS.pdf}
    \caption{NC}
    \label{fig:rq2_NC}
\end{subfigure}  
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_NULL_RETURNS.pdf}
    \caption{NRET}
    \label{fig:rq2_NRET}
\end{subfigure}

\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_INCREMENTS.pdf}
    \caption{INCR}
    \label{fig:rq2_INCR}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_EMPTY_RETURNS.pdf}
    \caption{ERET}
    \label{fig:rq2_ERET}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth, trim = 7mm 10mm 7mm 15mm]{figure/rq2/pie_FALSE_RETURNS.pdf}
    \caption{BFRET}
    \label{fig:rq2_BFRET}
\end{subfigure}

\caption{Mutators and Mutant status. CB, VMC and MATH are among the most useful mutators for initial surviving mutants, whereas NC, NRET, INCR, ERET, and BRET are those useful to generate killed mutants. 
}
\label{fig:rq2_mut_op_pie}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq2/Lang_chg.pdf}
    \caption{Lang}
    \label{fig:rq2_lang}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq2/Closure_chg.pdf}
    \caption{Closure}
    \label{fig:rq2_closure}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/rq2/total_chg.pdf}
    \caption{Total} % Or Josup
    \label{fig:rq2_total}
\end{subfigure}
\caption{Except for Lang, the pattern of revealing line being recently observed and relatively old frequently observed  %(overall, churn more frequent -> common)
}\label{fig:rq2_chg}
\end{figure}

\cref{tab:tab_rq2_mut_status} presents the general statistics of the final mutant status. Out of 12,239 surviving mutants we obtained, 10,383 remain after excluding ambiguous \fixme{will-survive}{}mutants inspected for less than 365 days and less interesting latent mutants that take more than 365 days to be detected. Note that we have propagated all 12,239 mutants but focus on this subset to avoid premature conclusions, taking those certain as discussed in \cref{subsub:mutant_status}. Among these 1,0383 mutants that we studied, a total of 3.5\% of them (i.e., 364) are latent, manifesting within 365 days after their introductions; most of these mutants either survive (48.7\%) or are dead (47.8\%) after the propagation. The exact percentage of the final status varies depending on the project. However, overall, only a small percentage of mutants are identified as latent across all projects.

\cref{tab:tab_rq2_rv_mut_mutop} shows which mutation operators are more likely to generate latent mutants than the others. Negate Conditionals (NC), which was the most effective in generating killed mutants, is also the most effective in creating latent mutants. Math, the third effective mutator for surviving mutants, follows the next. In fact, the mutators useful for latent mutants include effective mutators from both groups. This suggests that latent mutants lie somewhere between the initial surviving and killed, sharing characteristics with both. 

\fixme{}{include only five ops?} % Fig 3 might be too large and contain unimportant information as our focus is not on surviving and dead mutants. So, drop and include only the top five mostly used operators? 
The majority of propagated mutants either survive to the end or become lost, i.e., dead, during the propagation, as shown in \cref{tab:tab_rq2_mut_status}. \cref{fig:rq2_mut_op_pie} compares the proportions of latent, \fixme{surviving}{}, and dead mutants for the eight mutators selected from the set of effective mutators for initial surviving (3) and killed mutants (5). The pie charts in the figure show that the usage of different mutators leads to different characteristics of mutants; for instance, VMC tends to generate more mutants that remain undetected to the end. 

Previous analyses of the past change trends between initial surviving and killed mutants demonstrate that the past change trends of the mutated lines affect the detectability of mutants. We conducted the same analyses between latent, \fixme{surviving}{}, and dead mutants. For consistency, we include the results of the same projects studied in RQ1. The boxplots in \cref{fig:rq2_chg}. show that these three mutant types have different trends of past changes. Compared to the change trend we observed in \cref{fig:rq1_chg},, the projects that had different tendencies, such as Lang and Closure, now share a similar trend, mainly in the age of the mutated code ($age_{min}$ and $age_{max}$). We find out that latent mutants (i.e., green) often reside in the code relatively recently modified by developers and in fairly new lines or methods, compared to the mutants that have never been killed (i.e., orange). However, we also observe the opposite, similar to the previous comparison between the original surviving and killed mutants. The churn metric of the change frequency and the number of developers differ between mutant types and further between projects.
\cref{fig:rq2_total} presents the combined results of mutants across projects. Despite individual projects having their characteristics, shared trends exist between mutants across different projects: overall, latent mutants are found in the code that the developer modified or introduced relatively recently, compared to surviving and dead mutants.\footnote{note that for dead mutants, the trend is quite different from what has been found in individual projects. This is due to a certain project, in this case, Math, dominating the others by having a strong trend for dead mutants.}
%Overall, mutants injected to the recently changed or introduced code are often more likely to be later revealed, i.e., latent, than those in the 
%\fixme{For the change frequency and the number of developers, there }{drop?}

% tech-debt discussion
The changes that mutants go through may affect the final status of propagated mutants. The first columns of each change category in \cref{tab:tab_rq2_revealed_mutant_cat}  present the number of latent ($L$), surviving ($S$), and dead ($D$) mutants after the propagation. The 93\% of the mutants we investigated did not undergo any changes while being propagated, as shown in the \textit{NoChange} column; around half of these mutants survive to the end, and developers overwrite the other half (dead). The remaining 334 mutants are revealed in later commits. In fact, most of the latent mutants of all projects belong to this \textit{NoChange} and, thereby, NC$_{NC}$ category, except Collections, JacksonXml, and JxPath, where none are revealing. These observations imply that latent mutants are often uncovered by changes in dependent code rather than changes to the mutants themselves.
The \textit{Semantic} column of \cref{tab:tab_rq2_revealed_mutant_cat} further supports these findings. Despite containing only the mutants on the semantically changed code, the ratio of latent mutant (6.26\%) does not differ much from the ratio in NC$_{NC}$ (3.45\%). Only 15 mutants are purely refactored, and they are mainly from Lang. In our study, most of the mutants that underwent refactoring also underwent semantic changes: out of 524 mutants on the semantically changed code, 194 experienced code refactorings. These results imply that mutants are rarely revealed by code refactoring. 

\cref{tab:tab_rq2_revealed_mutant_cat} shows how many days it takes to detect latent mutants, in addition to the impact of change types on mutants. On average, latent mutants require 103.5 days to be caught by future test suites; this number increases to 344.8 days if we remove the threshold ($N_{thr}$) of 365 days. This means that developers can save the technical debt of about 100 days by having these latent mutants in advance. Regarding technical debt, mutants that underwent semantic changes have smaller debts than those that have never gone through any changes (NC). However, when we compare mutants based on whether the change directly affects the revealing status, denoted by the subscript $_C$ and $_{NC}$, latent mutants that are indirectly caught by the changes on dependent code have similar debt regardless of whether the mutated code has been semantically changed or not: 84.8 days for SC$_{NC}$ and 106.7 days for NC$_{NC}$. 

\noindent\textbf{Answer to RQ2:} Only around 3.5\% of the initial surviving mutants later manifest as latent mutants. Mutators effective in generating killed mutants are also useful in generating latent mutants, and similar holds for the surviving mutants, positioning the latent mutants somewhere between these two mutant groups. Latent mutants have different trends of past changes compared to those never caught and those overwritten, often residing in relatively recent code. Most of these mutants are detected by the propagated changes in dependent code, and their technical debt is about 100 days. 

\begin{table}[ht] 
\caption{Categorised mutants and their life span. L/NL/D refer to the number of latent, non-latent, and discarded mutants under each change type (i.e., \textit{Semantic}, \textit{Refactoring}, \textit{NoChange}). Remaining columns report the number of mutants and the average life-span ($dbt$) of change-based, five mutant types (days)
}\label{tab:tab_rq2_revealed_mutant_cat}
\scalebox{0.67}{
\begin{tabular}{lr|r|rrrrrr|r|rrrrrr|r|rr}
\toprule
& & \multicolumn{7}{c|}{Semantic (and Refactoring (194))}  & \multicolumn{7}{c|}{Refactoring} & \multicolumn{3}{c}{NoChange} \\
& & \#$_{mut}$ & \multicolumn{2}{c}{SC$_C$} & \multicolumn{2}{c}{SC$_{NC}$} & \multicolumn{2}{c|}{total} & \#$_{mut}$ & \multicolumn{2}{c}{RC$_C$} & \multicolumn{2}{c}{RC$_{NC}$} & \multicolumn{2}{c|}{total} & \#$_{mut}$ &\multicolumn{2}{c}{NC$_{NC}$}\\
%proj & \#$^{all}_{rev}$ & \#$_{mut}$ & \#$^{latent}_{mut}$/\#$^{surv}_{mut}$/\#$^{dead}_{mut}$ & \# & dbt & \# & dbt & \# & dbt & \#$^{latent}_{mut}$/\#$^{surv}_{mut}$/\#$^{dead}_{mut}$ & \# & dbt & \# & dbt & \# & dbt & \#$^{latent}_{mut}$/\#$^{surv}_{mut}$/\#$^{dead}_{mut}$ & \# & dbt \\
proj & \#$_{rev}$ & L/NL/D & \# & dbt & \# & dbt & \# & dbt & L/NL/D & \# & dbt & \# & dbt & \# & dbt & L/NL/D & \# & dbt \\
\midrule
Lang & 27 & 1/44/25 & 1 & 1.5 & 0 & 0.0 & 1 & 1.5 & 3/3/4 & 0 & 0.0 & 0 & 0.0 & 3 & 2.0 & 35/571/147 & 35 & 111.6\\
Math & 79 & 15/171/30 & 1 & 16.2 & 14 & 68.0 & 15 & 64.5 & 0/0/0 & -- & -- & -- & -- & -- & -- & 121/660/445 & 121 & 85.6\\
Time & 10 & 0/2/0 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 5/71/1 & 5 & 245.1\\
Closure & 100 & 0/29/1 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 33/1639/540 & 33 & 144.4\\
Cli & 22 & 0/10/0 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 10/174/38 & 10 & 4.2\\
Compress & 43 & 2/41/43 & 1 & 56.9 & 1 & 319.9 & 2 & 188.4 & 0/0/1 & -- & -- & -- & -- & -- & -- & 24/503/475 & 24 & 147.1\\
Codec & 16 & 2/20/5 & 2 & 2.6 & 0 & 0.0 & 2 & 2.6 & 0/0/0 & -- & -- & -- & -- & -- & -- & 11/128/105 & 11 & 53.7\\
Collections & 2 & 0/0/0 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 0/4/0 & -- & -- \\
Csv & 11 & 0/9/9 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 1/106/18 & 1 & 0.8\\
JacksonCore & 21 & 1/0/22 & -- & -- & -- & -- & -- & -- & 2/0/2 & 0 & 0.0 & 1 & 228.4 & 3 & 232.7 & 48/330/2230 & 48 & 150.2\\
JacksonXml & 3 & 0/0/0 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 0/4/13 & -- & -- \\
JxPath & 9 & 0/2/0 & -- & -- & -- & -- & -- & -- & 0/0/0 & -- & -- & -- & -- & -- & -- & 0/120/13 & -- & -- \\
Jsoup & 79 & 4/16/22 & 3 & 0.4 & 0 & 0.0 & 3 & 0.4 & 0/0/0 & 0 & 0.0 & 1 & 238.1 & 1 & 238.1 & 46/399/774 & 46 & 87.1\\
\midrule
Total & 422 & 25/344/157 & 8 & 10.1 & 15 & 84.8 & 23 & 58.8 & 5/3/7 & 0 & 0.0 & 2 & 233.3 & 7 & 134.6 & 334/4709/4799 & 334 & 106.7\\
\bottomrule
\end{tabular}}
\end{table}

%\begin{figure}[h]
%  \centering
%  \includegraphics[width=1.0\linewidth]{figure/rv_muts_pc_debt.pdf}
%  \caption{Technical Debt for each cateogry }
%  \label{fig:rq4_biseciton}
%\end{figure}

\subsection{RQ3. Latent Mutant Prediction} % (fold)
\label{sub:rq3_latent_mutant_prediction}



\cref{sub:rq2_revealed_mutants_characteristics} shows that only a small percentage of initial surviving mutants are latent, further emphasizing the need to predict these mutants. From the previous analyses of the mutant characteristics, we observe that latent mutants have different historical trends of changes compared to\textit{survive} and \textit{dead} mutants, and vice-versa; we also observe that the choice of mutation operators affects the mutant status. Thus, we use both eight historical metric features and mutation operators to train the classification model. \cref{tab:tab3_revealed_mutants} presents the classification results of the final mutant status, i.e., \textit{latent}, \textit{survive}, and \textit{dead},, using a Random Forest Classifier. We take the random prediction as our baseline to show that these latent mutants are identifiable. 

Overall, the RF classification model outperforms the random baseline, achieving an accuracy of 0.87 and a balanced accuracy of 0.67. For the accuracy per class within the parenthesis, in most cases, the model obtains an accuracy higher than 0.9 for the latent mutant class.\footnote{these class-wise values are often better than both accuracy and balanced accuracy, which takes the average of the sensitivity and specificity}.
While these accuracy values demonstrate that the classification can predict the final mutant status, they report the general prediction performance over all classes; as the latent mutant takes only an average of 3.5\% of the initial surviving mutants, these metrics may not be well-suited to compare the performance regarding the latent mutant identification. Hence, we compute another evaluation metric, Mean Average Precision (MAP). In this study, MAP is calculated as the mean of the average precision of all revisions, i.e., fixed commits, for each project. Here, we regard the latent mutants as the target to predict and compute the precision at each point in the list of mutants ranked in descending order of their likelihood to be latent. In the end, we define MAP as follows. 

\begin{equation}%
\scalebox{0.95}{  
MAP = $\frac{1}{\#_{rev}}\sum_{i = 1}^{M} \frac{Precision(i) \times isLatent(i)}{\# \text{of latent mutants}}\text{,  } Precision(i) = \frac{\#\text{ of latent mutants within the top i}}{i}$
}
\end{equation}

\noindent In this equation, \#$_{rev}$ refers to the number of revisions, and $M$ is the number of mutants under inspection for each revision. Thus, if a revision contains only latent mutants or none at all, we skip the computation and mark the case with "--". MAP simulates the use case where developers have a set of mutants and want to identify which one is latent. Overall, the RF model obtains higher MAP values than the random baselines; for projects such as Time and Codec, the model acquires a MAP greater than 0.8. From these results, we argue that latent mutants can be predicted using the historical features and the mutation operator. 

\cref{tab:tab3_fimp} presents the feature importance of the trained models. Overall, the age features have higher feature importance values than the other features. This result conforms with the previous findings of different change trends for different mutant types. While historical features explain the characteristics of mutated code, mutation operators describe the mutation itself. Since these two contain different information, we further investigate how the mutation operator affects the prediction by training another model without using mutation operator information (\textit{wo mutOp}). The middle column in \cref{tab:tab3_fimp} shows a slight yet constant decrease in the accuracy across projects. 

\noindent\textbf{Answer to RQ3.} Using the historical features and mutation operators, latent mutants are identifiable. Among the historical features, the age features have the highest feature ... 

\begin{table}[ht] 
\caption{Final mutant status prediction. All values in cells are reported in average. $L$, $NL$ and $D$ refer to latent, non-latent, and discarded mutants. 
}\label{tab:tab_rq3_revealed_mutants}
\scalebox{0.7}{
\begin{tabular}{lr|rrr|rrr|rrr}
\toprule
& & \multicolumn{3}{c|}{Random Forest} & \multicolumn{3}{c|}{Random Forest (wo mutOp)} & \multicolumn{3}{c}{Random} \\
proj & \#$_{rev}$ & acc (L/NL/D) & bal$_{acc}$ & MAP & acc (L/NL/D) & bal$_{acc}$ & MAP & acc (L/NL/D) & bal$_{acc}$ & MAP\\
\midrule 
Lang & 27 & 0.89 (0.94/0.91/0.92) & 0.65 & 0.37 & 0.84 (0.94/0.87/0.87) & 0.61 & 0.37 & 0.34 (0.65/0.42/0.6) & 0.33 & 0.33 \\
Math & 79 & 0.82 (0.9/0.86/0.89) & 0.67 & 0.35 & 0.82 (0.89/0.85/0.89) & 0.63 & 0.31 & 0.34 (0.64/0.48/0.56) & 0.34 & 0.29 \\
Time & 10 & 0.89 (0.95/0.89/0.94) & 0.38 & 0.92 & 0.89 (0.95/0.89/0.95) & 0.37 & 0.92 & 0.35 (0.68/0.39/0.64) & 0.39 & 0.25 \\
Closure & 100 & 0.83 (0.99/0.83/0.84) & 0.63 & 0.45 & 0.77 (0.98/0.77/0.79) & 0.52 & 0.31 & 0.34 (0.66/0.42/0.59) & 0.33 & 0.15 \\
Cli & 22 & 0.86 (0.94/0.87/0.92) & 0.64 & 0.42 & 0.85 (0.94/0.85/0.91) & 0.62 & 0.39 & 0.34 (0.66/0.41/0.61) & 0.35 & 0.45 \\
Compress & 43 & 0.79 (0.97/0.8/0.8) & 0.59 & 0.3 & 0.78 (0.97/0.79/0.79) & 0.58 & 0.23 & 0.34 (0.66/0.5/0.51) & 0.34 & 0.25 \\
Codec & 16 & 0.89 (0.97/0.91/0.9) & 0.73 & 0.83 & 0.9 (0.97/0.91/0.91) & 0.76 & 0.81 & 0.33 (0.65/0.48/0.53) & 0.34 & 0.18 \\
Collections & 2 & 0.98 (1.0/0.98/0.98) & 0.98 & - & 1.0 (1.0/1.0/1.0) & 1.0 & - & 0.38 (0.7/0.38/0.68) & 0.38 & - \\
Csv & 11 & 0.94 (0.99/0.95/0.94) & 0.6 & - & 0.96 (0.99/0.97/0.96) & 0.62 & - & 0.33 (0.66/0.4/0.61) & 0.29 & - \\
JacksonCore & 21 & 0.96 (0.98/0.98/0.96) & 0.71 & 0.28 & 0.96 (0.98/0.98/0.97) & 0.73 & 0.33 & 0.34 (0.66/0.63/0.39) & 0.34 & 0.08 \\
JacksonXml & 3 & 0.66 (1.0/0.66/0.66) & 0.77 & - & 0.76 (1.0/0.76/0.76) & 0.84 & - & 0.36 (0.69/0.58/0.45) & 0.36 & - \\
JxPath & 9 & 0.85 (1.0/0.86/0.86) & 0.62 & - & 0.85 (1.0/0.85/0.85) & 0.6 & - & 0.34 (0.67/0.37/0.64) & 0.32 & - \\
Jsoup & 79 & 0.84 (0.95/0.86/0.86) & 0.61 & 0.29 & 0.84 (0.95/0.87/0.87) & 0.6 & 0.26 & 0.34 (0.65/0.56/0.46) & 0.34 & 0.28 \\
\midrule
Total & 422 & 0.87 (0.96/0.88/0.89) & 0.67 & 0.34 & 0.85 (0.96/0.87/0.87) & 0.64 & 0.32 & 0.34 (0.66/0.51/0.51) & 0.34 & 0.13 \\
\bottomrule
\end{tabular}}
\end{table}

%\begin{figure}[ht]
%\centering
%\begin{subfigure}{0.4\textwidth}
%    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/pred_eval.pdf}
%    \caption{Balanced Accuracy}
%\end{subfigure}
%\begin{subfigure}{0.4\textwidth}
%    \includegraphics[width=\textwidth, trim = 5mm 10mm 5mm 0mm]{figure/pred_eval_map.pdf}
%    \caption{Mean Average Precision}
%\end{subfigure}
%\caption{
%}\label{fig:rq3_rf_pred}
%\end{figure}

\begin{table}[ht] 
\caption{Feature Importance. The results are reported per fold (five fold). The cell highlighted in blue contains feature with the highest feature importance values. Those within the top three are highlighted in green. 
%The last row contains the results of Spearman correlation analysis between the debt time and the feature. 
}\label{tab:tab3_fimp}
\scalebox{0.7}{
\begin{tabular}{l|rrrrrrrrr}
\toprule
fold & mutOp & l\_churn & l\_min\_age & l\_max\_age & l\_n\_authors & e\_churn & e\_min\_age & e\_max\_age & e\_n\_authors \\
\midrule
0 & 0.101 & 0.038 & \cellcolor{green!25}{0.161} & \cellcolor{green!25}{0.188} & 0.017 & 0.087 & 0.144 & \cellcolor{blue!25}{0.211} & 0.054\\
1 & 0.101 & 0.038 & \cellcolor{green!25}{0.162} & \cellcolor{green!25}{0.185} & 0.017 & 0.086 & 0.146 & \cellcolor{blue!25}{0.211} & 0.055\\
2 & 0.101 & 0.037 & \cellcolor{green!25}{0.159} & \cellcolor{green!25}{0.189} & 0.017 & 0.087 & 0.145 & \cellcolor{blue!25}{0.211} & 0.055\\
3 & 0.102 & 0.037 & \cellcolor{green!25}{0.162} & \cellcolor{green!25}{0.187} & 0.017 & 0.087 & 0.144 & \cellcolor{blue!25}{0.21} & 0.054\\
4 & 0.102 & 0.037 & \cellcolor{green!25}{0.16} & \cellcolor{green!25}{0.187} & 0.017 & 0.087 & 0.144 & \cellcolor{blue!25}{0.212} & 0.054\\
\bottomrule
\end{tabular}}
\end{table}



% plus, spearman corr with debt_time -> positively correalted
% or addiitonal analysis by shuffling each feature and train the model 


% subsection rq3_latent_mutnat_prediction (end)




















==> study.tex <==

\section{Exploration of Propagated Mutants: Research Questions}\label{sec:exploration_of_propagated_mutants}

This study aims at investigating the interplay between mutation testing and software evolution, defining and studying the impact of latent mutants whose existences are undetectable in the current version (i.e., survive) but later revealed as the software evolves. Thus, our main objectives are divided into two folds: 1) exploring the prevalence and the potential of latent mutants and 2) investigating their characteristics and ways to identify them based on historical information. We thus introduce the following three research questions: 

\subsection{RQ1. Prevalence and Characteristics of Surviving Mutants:\textit{how prevalent and different are surviving mutants?}}\label{sub:rq1}

This study is motivated by the relative lack of interest in mutants that remain undetected by the current test suite, i.e., survive, compared to those that are killed. Hence, before studying latent mutants, we first investigate how common surviving mutants are and how they differ from killable mutants by examining the mutation operators that frequently lead to surviving/killed mutants.  %These historical properties/features have been shown to be effective in computing the defect-proneness of code elements. 
As software evolves through developer's changes, we conjecture that analysing this past change trend of the injection point, i.e., mutated code, may provide hints on the detectability of mutants. 
Hence, we further inspect the history properties of the mutated code elements, mainly the metadata that describes the past change trends of the elements. We select three types of historical features, i.e., \textit{age}, \textit{churn} and \textit{developers}, shown to be effective in describing the past change tendencies of code elements concerning their likelihood of causing test failures~\cite{McI:2018:tse, Kamei2013aa,Sohn2021saner}. 

\begin{itemize}
    \item \textit{Age} measures how long the code element has been in the codebase. We measure two types of ages, i.e., the minimum ($age_{min}$) and the maximum ($age_{max}$): the former computes the time interval from the last change, whereas the latter calculates the interval from the first introduction of the code element. 
    \item \textit{Churn} evaluates how frequently changed the code element is, counting the number of past changes made to the code element. 
    \item \textit{Developers} is the number of unique developers that modified the code element. 
\end{itemize}

We compute these four features per line ($l$) and method ($m$), as the line granularity can be too fine-grained to capture the general trend~\cite{}. As a result, eight features are investigated in total: $age^l_{min}$, $age^l_{max}$, $churn^l$, $n^l_{dev}$ with the line granularity and $age^m_{min}$, $age^m_{max}$, $churn^m$, $n^m_{dev}$ with the method granularity. We compare the trend of these feature metrics between surviving and killed mutants. 

\subsection{RQ2. Characteristics and Usefulness of Latent Mutants: }\label{sub:rq2}
%What are the characteristics of mutants that are survived at the time of the injection but later revealed? What kind of characteristics do they share with killed and surived mutants? Can we further categorise them? 
Latent mutants are the subset of surviving mutants that can manifest as software changes. Hence, we first examine the proportion of latent mutants among surviving mutants. More precisely, we inspect the ratio of latent, surviving and dead mutants \fixme{defined in \cref{sec:methodolgy_and_terminology}}{}; this inspection is to get a general idea on how prevalent latent mutants are. 
We then investigate the characteristics of latent mutants with the same set of features, including mutation operators, used to compare the characteristics of surviving and killed mutants. Using this feature set, we study how latent mutants differ from or are similar to surviving mutants and killed mutants and further to \fixme{will-survive}{need-to-think} mutants and dead mutants. 
Next, we assess the potential usefulness of latent mutants by computing the technical debt they represent. The technical debt of a mutant is computed as the number of days from the injection to the revelation by test failure: \fixme{the more it takes to detect a latent mutant, the more ...}{complete} %These values demonstrate the future cost that mutant may save by exposing the aspects that the test suite may fail to capture. 
In \cref{sub:code_change_type_and_mutant_propgaation}, we categorise mutants into five groups by the final change status of the mutated line and whether they are revealed directly or indirectly by the changes, aiming to inspect the impact of changes on the revelation of mutants. Thus, in this research question, we further compare the ratio of latent mutants and their technical debt for each category. \fixme{We do not repeat the change feature and mutator operator analyses here since this categorisation represents another independent variable that may affect the revelation of mutants\footnote{Change feature analysis is excluded here, since these five categories already reflect the past change trend. The selection of mutation operators are independent from this categorisation}}{drop?} 

\subsection{RQ3. Latent Mutant Prediction: \textit{can we identify latent mutants among surviving mutants in advance?}}\label{sub:rq3}
We answer this research question by training a simple classifier that predicts the final labels of surviving mutants, i.e., latent, surviving, and dead, with the eight historical features and the mutation operators chosen to study the mutant characteristics in previous research questions. For the training algorithm, we select Random Forest (RF), which has often been employed to predict the defect-proneness of the code, i.e., the likelihood of causing a program failure, using the historical change features.~\cite{}. %We repeat the training 10 times to compensate the stochastic nature of RF. 
As the primary objective of this study lies in exploring the characteristics of latent mutants, we further investigate the feature importance of the trained model \fixme{to ..}{complete}
. %assess which feature contributes the most and o 




















